Differentially Private Federated Learning With Time-Adaptive Privacy Spending

Federated learning (FL) with differential privacy (DP) provides a framework for collaborative machine learning, enabling clients to train a shared model while adhering to strict privacy constraints. The framework allows each client to have an individual privacy guarantee, e.g., by adding different amounts of noise to each client's model updates. One underlying assumption is that all clients spend their privacy budgets uniformly over time (learning rounds). However, it has been shown in the literature that learning in early rounds typically focuses on more coarse-grained features that can be learned at lower signal-to-noise ratios while later rounds learn fine-grained features that benefit from higher signal-to-noise ratios. Building on this intuition, we propose a time-adaptive DP-FL framework that expends the privacy budget non-uniformly across both time and clients. Our framework enables each client to save privacy budget in early rounds so as to be able to spend more in later rounds when additional accuracy is beneficial in learning more fine-grained features. We theoretically prove utility improvements in the case that clients with stricter privacy budgets spend budgets unevenly across rounds, compared to clients with more relaxed budgets, who have sufficient budgets to distribute their spend more evenly. Our practical experiments on standard benchmark datasets support our theoretical results and show that, in practice, our algorithms improve the privacy-utility trade-offs compared to baseline schemes.

==> algorithm1.tex <==


\begin{algorithm}[H]
\caption{Differential Private Federated Averaging (DP-FedAvg)~\citep{mcmahan2017learning}}
\textbf{Inputs:} No. clients $N$, No. global rounds $T$, No. local iterations $L$, noise multiplier $\noisem$, clip norm $c$, sampling rate $q$, loss functions $\{\loss_n\}_{n\in [N]}$, local datasets $\{\train_n\}_{n\in [N]}$, learning rate $\lr$, batch size $\bs$ 
%\State \textbf{Results:} Final global model $\model^T$
\label{alg:dpfl}
\begin{algorithmic}[1]
\State \textbf{Initialize} global model $\model^0$
\For{each global round $t \in [T]$} 
\State $\gC^t \gets$ Sample clients with probability $q$.
\For{each client $n\in \gC^t$ in parallel}
\State $\tilde{\Delta}\model_n^t$ =  
\texttt{ClientUpdate}$\left(t, n,\model^{t-1}\right)$.
\EndFor
\State Aggregate $\tilde{\Delta}\model^t = \sum_{n\in \gC^t} \tilde{\Delta}\model_n^t$
\State Add noise $\tilde{\Delta}\model^t \gets \tilde{\Delta}\model^t + \gN(0,c^2\noisem^2\sI)$
\State Update $\model^{t} = \model^{t-1} + \frac{\tilde{\Delta}\model^t}{qN}$
\EndFor
\Statex
\end{algorithmic}
\textbf{Def} \texttt{ClientUpdate}$\left(t, n,\model^{t}, c_n\right)$
\begin{algorithmic}[1]
\State \textbf{Initialize} local model $\model_n^{t,0}=\model^t$
\For{local iteration $l \in [l]$}
\State $\{\batch_i\}_{i=1}^{|\train_n|/B} \gets$ Split $\train_n$ to size $B$ batches
\For{each batch $\batch_i$}
\State $\model_n^{t,l} = \model_n^{t,l-1}-\frac{\lr}{\bs}\sum_{(\rvx,y)\in \batch_i} \nabla\loss\left(\model_n^{t,l-1};(\rvx,y)\right)$
\EndFor
\EndFor
\State Compute $\Delta\model_n^t = \model_n^{t,L} - \model_n^{t,0}$
\State Clip $\tilde{\Delta}\model_n^{t} = \Delta\model_n^t\min\left(1,\frac{c}{\left\|\Delta\model_n^{t}\right\|_2}\right)$  
\State Return $\tilde{\Delta}\model_n^{t}$ 
\end{algorithmic}
\end{algorithm}


==> algorithm2.tex <==
\begin{algorithm}[H]
\caption{Individualized DP-FedAvg (IDP-FedAvg), a natural integration of IDP~\citep{boenisch2024have} to FL}
\textbf{Inputs:} No. clients $N$, No. global rounds $T$, No. local iterations $L$, local privacy budgets $\{\eps_n\}_{n\in [N]}$, average clip norm $c$, sampling rate $q$, loss functions $\{\loss_n\}_{n\in [N]}$, local datasets $\{\train_n\}_{n\in [N]}$, learning rate $\lr$, batch size $\bs$, probability of violating $\delta$ 
%\State \textbf{Results:} Final global model $\model^T$
\label{alg:idpfl}
\begin{algorithmic}[1]
\State $\noisem, \{c_n\}_{n\in [N]}=$\texttt{SetPrivacyParams}$\left(c, q, \{\eps_n\}_{n\in [N]}, T, \delta\right)$
\State \textbf{Initialize} global model $\model^0$
\For{each global round $t \in [T]$} 
\State $\gC^t \gets$ Sample clients with probability $q$.
\For{each client $n\in \gC^t$ in parallel}
\State $\tilde{\Delta}\model_n^t$ =  
\texttt{ClientUpdate}$\left(t, n,\model^{t-1}, c_n\right)$.
\EndFor
\State Aggregate $\tilde{\Delta}\model^t = \sum_{n\in \gC^t} \tilde{\Delta}\model_n^t$
\State Add noise $\tilde{\Delta}\model^t \gets \tilde{\Delta}\model^t + \gN(0,c^2\noisem^2\sI)$
\State Update $\model^{t} = \model^{t-1} + \frac{\tilde{\Delta}\model^t}{qN}$
\EndFor
\Statex
\end{algorithmic}
\textbf{Def} \texttt{ClientUpdate}$\left(t, n,\model^{t}, c_n\right)$
\begin{algorithmic}[1]
\State \textbf{Initialize} local model $\model_n^{t,0}=\model^t$
\For{local iteration $l \in [l]$}
\State $\{\batch_i\}_{i=1}^{|\train_n|/B} \gets$ Split $\train_n$ to size $B$ batches
\For{each batch $\batch_i$}
\State $\model_n^{t,l} = \model_n^{t,l-1}-\frac{\lr}{\bs}\sum_{(\rvx,y)\in \batch_i} \nabla\loss\left(\model_n^{t,l-1};(\rvx,y)\right)$
\EndFor
\EndFor
\State Compute $\Delta\model_n^t = \model_n^{t,L} - \model_n^{t,0}$
\State Clip $\tilde{\Delta}\model_n^{t} = \Delta\model_n^t\min\left(1,\frac{c_n}{\left\|\Delta\model_n^{t}\right\|_2}\right)$  
\State Return $\tilde{\Delta}\model_n^{t}$ 
\Statex
\end{algorithmic}
\textbf{Def} \texttt{SetPrivacyParams}$\left(c, q, \{\eps_n\}_{n\in [N]}, T, \delta\right)$
\begin{algorithmic}[1]
\For{each client $n \in [N]$}
\State Set local noise multiplier $\noisem_n=$\texttt{GetNoise}$\left(\eps_n,\delta, q, T\right)$
\EndFor
\State Compute $\noisem \gets \left(\frac{1}{N}\sum_{n\in [N]}\frac{1}{\noisem_n}\right)^{-1}$
\For{each client $n \in [N]$}
\State Set local clip norm $c_n=\frac{c\noisem}{\noisem_n}$
\EndFor
\State Return $\noisem, \{c_n\}_{n\in [N]}$
\end{algorithmic}
\end{algorithm}

==> algorithm3.tex <==


\begin{algorithm}[H]
\caption{Time-Adaptive IDP-FedAvg (TIDP-FedAvg)}
\textbf{Inputs:} No. clients $N$, No. global rounds $T$, No. local iterations $L$, local privacy budgets $\{\eps_n\}_{n\in [N]}$, sampling rate $q$, average clip norm $c$, modes $\{M_n^t \in\{0,1\}_{n\in [N], t\in [T]}$, sampling rates for saving mode $\{q_n\}_{n\in [N]}$, loss functions $\{\loss_n\}_{n\in [N]}$, local datasets $\{\train_n\}_{n\in [N]}$, learning rate $\lr$, batch size $\bs$, probability of violating $\delta$ 
\label{alg:tidpfl}
\begin{algorithmic}[1]
\State $q^t, \noisem^t, \{q_n^t, c_n^t\}_{n\in [N]}=$\texttt{SetPrivacyParams}$\left(c, q, \{q_n\}_{n\in [N]}, \{\eps_n\}_{n\in [N]}, \{M^t\}_{t\in [T]}, T, \delta\right)$
\State \textbf{Initialize} global model $\model^0$
\For{each global round $t \in [T]$} 
\State $\gC^t \gets$ Sample clients with probability $\{q_n^t\}$.
\For{each client $n\in \gC^t$ in parallel}
\State $\tilde{\Delta}\model_n^t$ =  
\texttt{ClientUpdate}$\left(t, n,\model^{t-1}, c_n^t\right)$.
\EndFor
\State Aggregate $\tilde{\Delta}\model^t = \sum_{n\in \gC^t} \tilde{\Delta}\model_n^t +  \sum_{n\in  [N]\backslash \gC^t} \gN\left(0,\frac{c^2(\noisem^t)^2}{N}\sI\right)$
\State Update $\model^{t} = \model^{t-1} + \frac{\tilde{\Delta}\model^t}{q^tN}$
\EndFor
\Statex
\end{algorithmic}
\textbf{Def} \texttt{ClientUpdate}$\left(t, n,\model^{t}, c_n, \noisem_n\right)$
\begin{algorithmic}[1]
\State \textbf{Initialize} local model $\model_n^{t,0}=\model^t$
\For{local iteration $l \in [l]$}
\State $\{\batch_i\}_{i=1}^{|\train_n|/B} \gets$ Split $\train_n$ to size $B$ batches
\For{each batch $\batch_i$}
\State $\model_n^{t,l} = \model_n^{t,l-1}-\frac{\lr}{\bs}\sum_{(\rvx,y)\in \batch_i} \nabla\loss\left(\model_n^{t,l-1};(\rvx,y)\right)$
\EndFor
\EndFor
\State Compute $\Delta\model_n^t = \model_n^{t,L} - \model_n^{t,0}$
\State Clip $\tilde{\Delta}\model_n^{t} = \Delta\model_n^t\min\left(1,\frac{c_n}{\left\|\Delta\model_n^{t}\right\|_2}\right)$  
\State Add noise $\tilde{\Delta}\model_n^t \gets \tilde{\Delta}\model_n^t + \gN\left(0,\frac{c_n^2(\noisem_n^t)^2}{N}\sI\right)$
\State Return $\tilde{\Delta}\model_n^{t}$ 
\Statex
\end{algorithmic}
\textbf{Def} \texttt{SetPrivacyParams}$\left(c, q,  \{q_n\}_{n\in [N]}, \{\eps_n\}_{n\in [N]}, \{M_n^t\}_{n\in [N], t\in [T]}, T, \delta\right)$
\begin{algorithmic}[1]
\State \textbf{Initialize} $\eps_n^0 = \eps_n$  and $\eps_{\text{rdp},n}^{0}=0$
for all $n\in [N]$
\For{each global round $t\in [T]$}
\For{each client $n \in [N]$}
\State Set local noise multiplier $\noisem_n^t=$\texttt{GetNoise}$\left(\eps_n^{t-1},\delta, q, T-t\right)$
\State \textbf{If} $M_n^t=0$, \textbf{then} $q_n^t = q_n$, \textbf{Else}, $q_n^t = q$.
\State $\eps_{\text{rdp},n}^t=\eps_{\text{rdp},n}^{t-1}+$\texttt{Compute\_rdp}$\left(q_n^t,\noisem_n^t, \alpha\right)$
\State $\eps_n^t=\eps_n-$\texttt{get\_privacy\_spent}$\left(\alpha, \eps_{\text{rdp},n}^t,\delta\right)$
\EndFor
\State Compute $\noisem^t \gets \left(\frac{1}{N}\sum_{n\in [N]}\frac{1}{\noisem_n^t}\right)^{-1}$
\For{each client $n \in [N]$}
\State Set local clip norm $c_n^t=\frac{c\noisem^t}{\noisem_n^t}$
\EndFor
\EndFor
\State $q^t = \frac{1}{N} \sum_{n=1}^N q_n^t$
\State Return $q^t, \noisem, \{q_n^t, c_n^t\}_{n\in [N]}$
\end{algorithmic}
\end{algorithm}

==> algorithm3_adaclip.tex <==
\begin{minipage}{0.47\textwidth} 
\include{algorithm1_adaclip}
\end{minipage}%
\hspace{1em} 
\begin{minipage}{0.50\textwidth}  %
  \raggedright  % Left-align
 \begin{algorithm}[H]
   \scriptsize
\caption{Our Time-adaptive DP-FL Framework, integrated with Adaptive Clipping}
\textbf{Inputs:} No. clients $N$, No. global rounds $T$, No. local iterations $L$, local privacy budgets $\eps_n$, sampling rate $q$, average clip norm $c$, modes $M_n^t \in\{0,1\}$, sampling rates for saving mode $q_n$, loss functions $\loss_n$, datasets $\train_n$, learning rate $\lr$, batch size $\bs$, probability of violating $\delta$, $\gamma$ quantile, clip-related learning rate $\lr_\text{b}$ \\ 
\label{alg:tidpfl:train}
\begin{algorithmic}[1]
\State \textbf{Initialize} global model $\model^0$, $c^1 = c$
\State \textbf{Initialize} $\eps_n^0 = \eps_n$  and $\bar{\eps}_{\text{rdp},n}^0=0$ for all $n\in [N]$
\For{each global round $t \in [T]$} 
\State \tcb{$q^t, \noisem^t, \{q_n^t, c_n^t, \noisem_n^t, \eps_n^{t}, \bar{\eps}_{\text{rdp},n}^{t}\}_{n\in [N]}$\ $=$\texttt{SetParams}$\left(c^t, q,  \{q_n, M_n^t, \eps_n^{t-1}, \bar{\eps}_{\text{rdp},n}^{t-1}\}_{n\in [N]}, T, \delta, t \right)$}
\State $\gC^t \gets$ Sample clients with probability $\{q_n^t\}$.
\For{each client $n\in [N]$ in parallel}
\State $(b_n^t,\tilde{\Delta}\model_n^t)$ =  
\texttt{ClientUpdate}$\left(t, n,\model^{t-1}, c_n^t, \noisem_n^t, c^t\right)$.
\State
\EndFor
\State $\tilde{\Delta}\model^t = \sum_{n\in \gC^t} \tilde{\Delta}\model_n^t +  \sum_{n\in  [N]\backslash \gC^t} \gN\left(0,\frac{c^2(\noisem^t)^2}{N}\sI\right)$
\State Update $\model^{t} = \model^{t-1} + \frac{\tilde{\Delta}\model^t}{q^tN}$
\State \tcb{$c^{t+1}$=\texttt{SetClippig}$\left(\{b_n^t\}_{n\in \gC^t}, \noisem_{\text{b}},q, \gamma, \lr_{\text{b}}, c^t\right)$}
\EndFor
\Statex
\end{algorithmic}
\textbf{Def} \texttt{ClientUpdate}$\left(t, n,\model^{t}, c_n^t, \noisem_n^t, c^t\right)$
\begin{algorithmic}[1]
\State \textbf{Initialize} local model $\model_n^{t,0}=\model^t$
\For{local iteration $l \in [l]$}
\State $\{\batch_i\}_{i=1}^{|\train_n|/B} \gets$ Split $\train_n$ to size $B$ batches
\For{each batch $\batch_i$}
\State $\model_n^{t,l} = \model_n^{t,l-1}-\frac{\lr \sum_{(\rvx,y)\in \batch_i} \nabla\loss_n\left(\model_n^{t,l-1};(\rvx,y)\right)}{\bs}$
\EndFor
\EndFor
\State Compute $\Delta\model_n^t = \model_n^{t,L} - \model_n^{t,0}$
\State \tcb{Compute $b = \gI_{\left\|\Delta\model_n^t \right\|\leq c^t}$}
\State Clip $\tilde{\Delta}\model_n^{t} = \Delta\model_n^t\min\left(1,\frac{c_n^t}{\left\|\Delta\model_n^{t}\right\|_2}\right)$  
\State Add noise $\tilde{\Delta}\model_n^t \gets \tilde{\Delta}\model_n^t + \gN\left(0,\frac{(c_n^t)^2(\noisem_n^t)^2}{N}\sI\right)$
\State \tcb{Return $b, \tilde{\Delta}\model_n^{t}$} 
\Statex
\end{algorithmic}
\textbf{Def} \texttt{SetParams}$\left(c, q,  \{q_n, M_n^t, \eps_n^{t-1}, \bar{\eps}_{\text{rdp},n}^{t-1}\}_{n\in [N]}, T, \delta, t \right)$
\begin{algorithmic}[1]
%\State \textbf{Initialize} $\eps_n^0 = \eps_n$  and $\bar{\eps}_{\text{rdp},n}^0=0$ for all $n\in [N]$
%\For{each global round $t\in [T]$}
\For{each client $n \in [N]$}
\State  $\bar{\noisem}_n^t=$\texttt{GetNoise}$\left(\eps_n^{t-1},\delta, q, T-t\right)$
\State \tcb{$\noisem_n^t = \left(\frac{1}{(\bar{\noisem}_n^t)^{2}} - \frac{1}{(2\noisem_{\text{b}})^2}\right)^{-1/2}$}
\State \textbf{If} $M_n^t=0$, \textbf{then} $q_n^t = q_n$, \textbf{Else}, $q_n^t = q$.
\State $\reps{n}^t=$\texttt{Compute\_rdp}$\left(q_n^t,\bar{\noisem}_n^t, \alpha\right)$
\State $\bar{\eps}_{\text{rdp},n}^t = \bar{\eps}_{\text{rdp},n}^{t-1} +  \reps{n}^t$
\State $\eps_n^t=\eps_n-$\texttt{get\_privacy\_spent}$\left(\alpha, \bar{\eps}_{\text{rdp},n}^t,\delta\right)$
\EndFor
\State Compute $\noisem^t \gets \left(\frac{1}{N}\sum_{n\in [N]}\frac{1}{\noisem_n^t}\right)^{-1}$
\For{each client $n \in [N]$}
\State Set local clip norm $c_n^t=\frac{c\noisem^t}{\noisem_n^t}$
\EndFor
\State $q^t = \frac{1}{N} \sum_{n=1}^N q_n^t$
%\EndFor
\State \tcb{Return $q^t, \noisem^t, \{q_n^t, c_n^t, \noisem_n^t, \eps_n^{t}, \bar{\eps}_{\text{rdp},n}^{t}\}_{n\in [N]}$}
\Statex
\end{algorithmic}
\tcb{
\textbf{Def} \texttt{SetClippig}$\left(\{b_n^t\}_{n\in \gC^t}, \noisem_{\text{b}},q, \gamma, \lr_{\text{b}}, c^t\right)$}
\begin{algorithmic}[1]
\State \tcb{Aggregate $\tilde{b}^t = \sum_{n\in \gC^t} b_n^t$}
\State \tcb{Add noise $\tilde{b}^t \gets \tilde{b}^t + \gN(0,\noisem_{\text{b}}^2\sI)$ }
\State \tcb{Average $\tilde{b}^t \gets \frac{1}{qN}\tilde{b}^t $}
\State \tcb{Update $c^{t+1}=c^t \exp \left(-\lr_{\text{b}}
(\tilde{b}^t-\gamma)\right)$}
\State \tcb{Return $c^{t+1}$}
\end{algorithmic}
\end{algorithm}
\end{minipage}

==> algorithm3_privacy.tex <==


\begin{algorithm}[H]
\caption{The \algasgo Method in Our Time-adaptive DP-FL Framework}
\textbf{Inputs:} No. clients $N$, No. global rounds $T$, local privacy budgets $\{\eps_n\}_{n\in [N]}$, sampling rate $q$, average clip norm $c$, modes $\{M_n^t \in\{0,1\}\}_{n\in [N], t\in [T]}$, sampling rates for saving mode $\{q_n\}_{n\in [N]}$, probability of violating $\delta$. \\ \\ 
\label{alg:tidpfl:privacy}
\textbf{Def} \texttt{SetPrivacyParams}$\left(c, q,  \{q_n\}_{n\in [N]}, \{\eps_n\}_{n\in [N]}, \{M_n^t\}_{n\in [N], t\in [T]}, T, \delta\right)$
\begin{algorithmic}[1]
\State \textbf{Initialize} $\eps_n^0 = \eps_n$  and $\bar{\eps}_{\text{rdp},n}^0=0$
for all $n\in [N]$
\For{each global round $t\in [T]$}
\For{each client $n \in [N]$}
\State Set local noise multiplier $\noisem_n^t=$\texttt{GetNoise}$\left(\eps_n^{t-1},\delta, q, T-t\right)$
\State \textbf{If} $M_n^t=0$, \textbf{then} $q_n^t = q_n$, \textbf{Else}, $q_n^t = q$.
\State $\reps{n}^t=$\texttt{Compute\_rdp}$\left(q_n^t,\noisem_n^t, \alpha\right)$
\State $\bar{\eps}_{\text{rdp},n}^t = \bar{\eps}_{\text{rdp},n}^{t-1} +  \reps{n}^t$
\State $\eps_n^t=\eps_n-$\texttt{get\_privacy\_spent}$\left(\alpha, \bar{\eps}_{\text{rdp},n}^t,\delta\right)$
\EndFor
\State Compute $\noisem^t \gets \left(\frac{1}{N}\sum_{n\in [N]}\frac{1}{\noisem_n^t}\right)^{-1}$
\For{each client $n \in [N]$}
\State Set local clip norm $c_n^t=\frac{c\noisem^t}{\noisem_n^t}$
\EndFor
\EndFor
\State $q^t = \frac{1}{N} \sum_{n=1}^N q_n^t$
\State Return $q^t, \noisem, \{q_n^t, c_n^t\}_{n\in [N]}$
\end{algorithmic}
\end{algorithm}

==> algorithm3_training.tex <==


\begin{algorithm}[H]
\caption{Iterative Training in Our Time-adaptive DP-FL Framework}
\textbf{Inputs:} No. clients $N$, No. global rounds $T$, No. local iterations $L$, local privacy budgets $\{\eps_n\}_{n\in [N]}$, sampling rate $q$, average clip norm $c$, modes $\{M_n^t \in\{0,1\}\}_{n\in [N], t\in [T]}$, sampling rates for saving mode $\{q_n\}_{n\in [N]}$, loss functions $\{\loss_n\}_{n\in [N]}$, local datasets $\{\train_n\}_{n\in [N]}$, learning rate $\lr$, batch size $\bs$, probability of violating $\delta$ 
\label{alg:tidpfl:train}
\begin{algorithmic}[1]
\State $q^t, \noisem^t, \{q_n^t, c_n^t\}_{n\in [N]}=$\texttt{SetPrivacyParams}$\left(c, q, \{q_n\}_{n\in [N]}, \{\eps_n\}_{n\in [N]}, \{M^t\}_{t\in [T]}, T, \delta\right)$
\State \textbf{Initialize} global model $\model^0$
\For{each global round $t \in [T]$} 
\State $\gC^t \gets$ Sample clients with probability $\{q_n^t\}$.
\For{each client $n\in \gC^t$ in parallel}
\State $\tilde{\Delta}\model_n^t$ =  
\texttt{ClientUpdate}$\left(t, n,\model^{t-1}, c_n^t\right)$.
\EndFor
\State Aggregate $\tilde{\Delta}\model^t = \sum_{n\in \gC^t} \tilde{\Delta}\model_n^t +  \sum_{n\in  [N]\backslash \gC^t} \gN\left(0,\frac{c^2(\noisem^t)^2}{N}\sI\right)$
\State Update $\model^{t} = \model^{t-1} + \frac{\tilde{\Delta}\model^t}{q^tN}$
\EndFor
\Statex
\end{algorithmic}
\textbf{Def} \texttt{ClientUpdate}$\left(t, n,\model^{t}, c_n, \noisem_n\right)$
\begin{algorithmic}[1]
\State \textbf{Initialize} local model $\model_n^{t,0}=\model^t$
\For{local iteration $l \in [l]$}
\State $\{\batch_i\}_{i=1}^{|\train_n|/B} \gets$ Split $\train_n$ to size $B$ batches
\For{each batch $\batch_i$}
\State $\model_n^{t,l} = \model_n^{t,l-1}-\frac{\lr}{\bs}\sum_{(\rvx,y)\in \batch_i} \nabla\loss\left(\model_n^{t,l-1};(\rvx,y)\right)$
\EndFor
\EndFor
\State Compute $\Delta\model_n^t = \model_n^{t,L} - \model_n^{t,0}$
\State Clip $\tilde{\Delta}\model_n^{t} = \Delta\model_n^t\min\left(1,\frac{c_n}{\left\|\Delta\model_n^{t}\right\|_2}\right)$  
\State Add noise $\tilde{\Delta}\model_n^t \gets \tilde{\Delta}\model_n^t + \gN\left(0,\frac{c_n^2(\noisem_n^t)^2}{N}\sI\right)$
\State Return $\tilde{\Delta}\model_n^{t}$ 
\Statex
\end{algorithmic}
\end{algorithm}

==> macros.tex <==
% include in main: \input{macros}

\usepackage{xparse}
\usepackage{xspace}
%\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{algorithm}% http://ctan.org/pkg/algorithm
\usepackage{algpseudocode}% http://ctan.org/pkg/algorithmicx
\usepackage{fixltx2e}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{tikz}
\usepackage{float}
\usepackage{multirow}
\usepackage{multicol}
%\usepackage{todonotes}
\usepackage{colortbl}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables
\usepackage{bbm}
\usepackage[shortlabels]{enumitem}
\usepackage[tiny]{todonotes}

\usepackage{hyperref,amssymb,enumitem}

\usepackage{wrapfig}

\usepackage{cleveref}

% Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

\setlist[itemize]{leftmargin=*}
\setlist[enumerate]{leftmargin=*}

%%%%%%%%%%%%%%%%%%%%%%%%%%

%\floatname{algorithm}{Procedure}
\renewcommand{\algorithmicrequire}{\textbf{Input: }}

\renewcommand{\algorithmicensure}{\textbf{Output: }}

\newcommand{\ie}{\textit{i.e.,}\@\xspace}
\newcommand{\eg}{\textit{e.g.,}\@\xspace}
\newcommand{\etal}{\textit{et al.}\@\xspace}

\newcommand{\aug}{\text{Aug}}

\newcommand{\Aug}{\text{Aug}}

\newcommand{\lalign}{\mathcal{L}_{\text{align}}}
\newcommand{\Halign}{\mathcal{H}_{\text{align}}}

\newcommand{\alignexp}[2]%{\mathbb{E}_{{#2}', {#2}'' \sim \Aug(x) } d({#1}({#2}'), {#1}({#2}'')) }
{\underset{ {#2}', {#2}'' \sim \Aug(x) }{\mathbb{E}} [ d\left({#1}({#2}'), {#1}({#2}'')\right) ] }


\newcommand{\dmetric}[2]{d({#1},{#2})}

\newcommand{\pr}{\mathbf{Pr}}
\newcommand{\dist}{\mathcal{D}}
\newcommand{\err}{\text{err}}

\newcommand{\upi}{^{(i)}}
\newcommand{\enc}{f_v}

\newcommand{\canary}{candidate\xspace}
\newcommand{\canaries}{candidates\xspace}
\newcommand{\method}{method\xspace}
\newcommand{\methods}{methods\xspace}
\newcommand{\Method}{method\xspace}
\newcommand{\Methods}{methods\xspace}
\newcommand{\name}{\texttt{SSLMem}\xspace}

% Secure Multi-party Computation
\newcommand{\smc}{MPC\xspace}
\newcommand{\single}{single-label\xspace}
\newcommand{\multi}{multi-label\xspace}
\usepackage{amsmath}

\DeclareRobustCommand\encircle[1]{\tikz[baseline=(char.base)]{\node[shape=circle,fill,inner sep=1pt] (char) {\textcolor{white}{#1}}}}

%\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1}

% ATTACKS
\newcommand{\Jacobian}{Jacobian\xspace}
\newcommand{\DataFree}{DataFree\xspace}
\newcommand{\JacobianTR}{Jacobian-TR\xspace}


% Abbreviations.
\newcommand{\IND}{IND\xspace} % IN-Distribution 

% Adam's commands:
%\newcommand{\myitem}{\paragraph}
\newcommand{\myitem}{\textbf}
\newcommand{\badX}{100x\xspace}

   
% \usepackage[backend=biber,style=numeric,citestyle=numeric,sorting=none]{biblatex}
% \DeclareMathOperator*{\Argmin}{argmin}
% \DeclareMathOperator*{\Argmax}{argmax}
% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{fact}[theorem]{Fact}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{notation}[theorem]{Notation}
% \newtheorem{assumption}{Assumption}


\graphicspath{{images/}}

\newif\ifdraft
\drafttrue

\newcommand\classratesize{0.8}

%Source: https://tex.stackexchange.com/questions/85200/include-data-from-a-txt-verbatim

\usepackage{fancyvrb}

% redefine \VerbatimInput
\RecustomVerbatimCommand{\VerbatimInput}{VerbatimInput}%
{fontsize=\footnotesize,
 %
 frame=lines,  % top and bottom rule only
 framesep=2em, % separation between frame and text
 %rulecolor=\color{Gray},
 %
% label=\fbox{\color{Black}data.txt},
% labelposition=topline,
 %
 commandchars=\|\(\), % escape character and argument delimiters for
                      % commands within the verbatim
 commentchar=*        % comment character
}

% COMMENTS
\ifdraft
\newcommand{\mynote}[1]{\textcolor{red}{[note: #1]}}
\newcommand{\franzi}[1]{\textcolor{purple}{[Franzi: #1]}}

\else
\newcommand{\franzi}[1]{}




